SuperDec: 3D Scene Decomposition with Superquadric Primitives

We present SuperDec, an approach for creating compact 3D scene representations via decomposition into superquadric primitives. While most recent works leverage geometric primitives to obtain photorealistic 3D scene representations, we propose to leverage them to obtain a compact yet expressive representation. We propose to solve the problem locally on individual objects and leverage the capabilities of instance segmentation methods to scale our solution to full 3D scenes. In doing that, we design a new architecture which efficiently decompose point clouds of arbitrary objects in a compact set of superquadrics. We train our architecture on ShapeNet and we prove its generalization capabilities on object instances extracted from the ScanNet++ dataset as well as on full Replica scenes. Finally, we show how a compact representation based on superquadrics can be useful for a diverse range of downstream applications, including robotic tasks and controllable visual content generation and editing.

==> macros.tex <==
%% ----------------------------------------------------------------------------
% CVG SA/MA thesis template
%
% Created 03/08/2024 by Tobias Fischer
%% ----------------------------------------------------------------------------
\ProvidesPackage{mydefs}
\usepackage{graphicx,calc} % for pix
% \usepackage{subfigure}
\usepackage{color}    % for colored text
\usepackage{ifthen}
\usepackage{paralist}
\usepackage{times}
\usepackage{longtable}
\usepackage{colortbl}
\usepackage{nomencl}
\usepackage{mathtools}
\usepackage{booktabs}
\usepackage{overpic}
\usepackage{xcolor}

\usepackage[dvipsnames]{xcolor}

\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepackage{filecontents}

% \renewcommand{\vec}[1]{\mathbf{#1}}
% \newcommand{\mat}[1]{\mathtt{#1}}
% \newcommand{\pinv}{^{+}}
% \newcommand{\inv}{^{-1}}
% \newcommand{\trans}{^{\!\top}}
% \newcommand{\invtrans}{^{-\!\top}}
% \newcommand{\myref}[1]{(\ref{#1})}
% \newcommand{\myeqref}[1]{Eq.~\myref{#1}}
% \newcommand{\myfigref}[1]{Fig.~\ref{#1}}
% \newcommand{\mychapterref}[1]{Chapter~\ref{#1}}
% \newcommand{\mysecref}[1]{Section~\ref{#1}}
% \newcommand{\myalgoref}[1]{Algorithm~\ref{#1}}
% \newcommand{\ie}{\textit{i.e.}}
% \newcommand{\eg}{\textit{e.g.}}
% \newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}

%--------Basic Math--------
% \NewDocumentCommand{\floor}{m}{\left\lfloor #1 \right\rfloor}
% \NewDocumentCommand{\ceil}{m}{\left\lceil #1 \right\rceil}
% \NewDocumentCommand{\ip}{m}{\left\langle #1 \right\rangle}

% \newcommand*{\abs}[1]{\left| #1 \right|}
% \newcommand*{\card}[1]{\left| #1 \right|}
% \NewDocumentCommand{\norm}{sm}{\IfBooleanTF{#1}{\|#2\|}{\left\| #2 \right\|}}

\newcommand*{\defeq}{\vcentcolon=}
\newcommand*{\eqdef}{=\vcentcolon}
\newcommand*{\lr}{\eta}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\dif}[2]{\frac{d#1}{d#2}}
\newcommand{\pd}[2]{\frac{\partial#1}{\partial#2}}

\usepackage{pifont}% http://ctan.org/pkg/pifont

\DeclareMathOperator*{\almostsurely}{\overset{a.s.}{\rightarrow}}
\DeclareMathOperator*{\eqalmostsurely}{\overset{a.s.}{=}}
\DeclareMathOperator*{\convp}{\overset{\fnPr}{\rightarrow}}
\DeclareMathOperator*{\convd}{\overset{\mathcal{D}}{\rightarrow}}
\DeclareMathOperator*{\convms}{\overset{\ell_2}{\rightarrow}}


\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
%------Functions-------
\newcommand{\sign}[1]{\text{sign}\left( #1 \right)}
\renewcommand*{\exp}[1]{\text{exp}\left( #1 \right)}
\renewcommand*{\sin}[1]{\text{sin}\left( #1 \right)}
\renewcommand*{\cos}[1]{\text{cos}\left( #1 \right)}
\newcommand*{\sigmoid}[1]{\sigma\left( #1 \right)}
\newcommand*{\sample}[2]{#1^{(#2)}} %sample #2-th of the dataset #1
\newcommand*{\layeru}[2]{#1^{[#2]}} %layer #2-th of the dataset #1 (upper)
\newcommand*{\layerl}[2]{#1_{[#2]}} %layer #2-th of the dataset #1 (lower)
\newcommand*{\epochu}[2]{#1^{\{#2\}}} %epoch #2-th using the dataset #1 (upper)
\newcommand*{\epochut}[2]{#1^{\{#2\}^\top}} %epoch #2-th using the dataset #1 (upper transpose)
\newcommand*{\epochl}[2]{#1_{\{#2\}}} %epoch #2-th using the dataset #1 (lower)
\newcommand*{\timeu}[2]{#1^{#2}}
\newcommand*{\timel}[2]{#1_{#2}}
\newcommand*{\loss}{\mathcal{L}}
\newcommand*{\dataset}{\mathbb{D}}

%--------Sets--------
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Rzero}{\mathbb{R}_{\geq 0}}
\newcommand{\Nat}{\mathbb{N}}
\newcommand{\NatZ}{\mathbb{N}_0}


%--------Names--------
\newcommand{\MSE}{\mathrm{MSE}}
\newcommand{\MLE}{\mathrm{MLE}}
\newcommand{\MAP}{\mathrm{MAP}}
\newcommand{\train}{\mathrm{train}}
\newcommand{\val}{\mathrm{val}}
\newcommand{\id}{\mathrm{id}}


%--------Symbols--------
\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\rvec}[1]{\mathbf{#1}}
\newcommand{\set}[1]{\mathbf{\uppercase{#1}}}
\newcommand{\spa}[1]{\mathcal{#1}}
\newcommand{\data}{\mathcal{D}}


\newcommand{\mean}[1]{\overline{#1}}
\newcommand{\compl}[1]{\overline{#1}}

%--------Operators--------
\NewDocumentCommand{\Ind}{m}{\mathds{1}\{{#1}\}}
\NewDocumentCommand{\fnPr}{}{\mathbb{P}}
\RenewDocumentCommand{\Pr}{om}{\fnPr\IfValueT{#1}{_{#1}}\parentheses*{#2}}
%\RenewDocumentCommand{\H}{mo}{H\IfValueTF{#2}{\left[#1\ \middle|\ #2\right]}{\brackets*{#1}}}
%\NewDocumentCommand{\Hsm}{mo}{H\IfValueTF{#2}{[#1 \mid #2]}{\brackets{#1}}}
%\NewDocumentCommand{\I}{mmo}{I\IfValueTF{#3}{\!\left(#1;#2\ \middle|\ #3\right)}{\parentheses*{#1; #2}}}
%\NewDocumentCommand{\Ism}{mmo}{I\IfValueTF{#3}{\!(#1;#2 \mid #3)}{\parentheses{#1; #2}}}
%\NewDocumentCommand{\fnS}{}{S}
%\RenewDocumentCommand{\S}{m}{\fnS\brackets*{#1}}
\newcommand{\Exp}[2]{\mathbb{E}_{#1}\brackets*{#2}}
\newcommand{\ExpS}[1]{\mathbb{E}_{#1}}
\NewDocumentCommand{\E}{somo}{\ensuremath{\mathbb{E}\IfValueT{#2}{_{#2}}{} \IfBooleanTF{#1}{#3}{\IfValueTF{#4}{\left[#3\ \middle|\ #4\right]}{\brackets*{#3}}}}}
\NewDocumentCommand{\Cov}{som}{\mathrm{Cov}\IfValueT{#2}{_{#2}}{} \IfBooleanTF{#1}{#3}{\brackets*{#3}}}
\NewDocumentCommand{\KL}{mm}{D_{\text{KL}}\parentheses*{#1 \| #2}}

\NewDocumentCommand{\pset}{m}{\mathcal{P}\parentheses*{#1}}

\newcommand{\grad}[2]{\boldsymbol{\nabla}_\vec{#2}#1}
\NewDocumentCommand{\jac}{}{\mD}
\NewDocumentCommand{\hes}{}{\mH}
\NewDocumentCommand{\BigO}{m}{\mathcal{O}\parentheses*{#1}}
\NewDocumentCommand{\BigOTil}{m}{\mathcal{O}^*\parentheses*{#1}}

%------Matrix and Vector------
% \NewDocumentCommand{\transpose}{m}{#1^\top}
\NewDocumentCommand{\inv}{m}{#1^{-1}}
\RenewDocumentCommand{\det}{m}{\mathrm{det}\parentheses*{#1}}
\NewDocumentCommand{\tr}{m}{\mathrm{tr}\parentheses*{#1}}
\NewDocumentCommand{\diag}{m}{\text{diag}(\vec{#1})}
\NewDocumentCommand{\msqrt}{m}{#1^{\nicefrac{1}{2}}}
\NewDocumentCommand{\vecop}{m}{\mathrm{vec}\brackets{#1}}

%--------Probability--------
\NewDocumentCommand{\N}{omm}{\mathcal{N}(\IfValueT{#1}{#1;}{} #2, #3)}
\NewDocumentCommand{\SN}{o}{\mathcal{N}(\IfValueT{#1}{#1;}{} \vzero, \mI)}
\NewDocumentCommand{\uSN}{o}{\mathcal{N}(\IfValueT{#1}{#1;}{} 0, 1)}
\NewDocumentCommand{\KF}{ommmmm}{\mathcal{KF}(\IfValueT{#1}{#1;}{} #2, #3, #4, #5, #6)}
\NewDocumentCommand{\GP}{omm}{\mathcal{GP}(\IfValueT{#1}{#1;}{} #2, #3)}
\NewDocumentCommand{\Unif}{om}{\mathrm{Unif}(\IfValueT{#1}{#1;}{} #2)}
\NewDocumentCommand{\Bern}{om}{\mathrm{Bern}(\IfValueT{#1}{#1;}{} #2)}
\NewDocumentCommand{\Bin}{omm}{\mathrm{Bin}(\IfValueT{#1}{#1;}{} #2, #3)}
\NewDocumentCommand{\Beta}{omm}{\mathrm{Beta}(\IfValueT{#1}{#1;}{} #2, #3)}
\NewDocumentCommand{\Laplace}{omm}{\mathrm{Laplace}(\IfValueT{#1}{#1;}{} #2, #3)}

%--------Common vectors/matrices/sets--------
\newcommand{\accessVectorAt}[2]{#1[#2]}
\newcommand{\accessMatrixAt}[3]{#1[#2][#3]}

\newcommand{\vzero}{\vec{0}}
\newcommand{\vone}{\vec{1}}
\newcommand{\va}{\vec{a}}
\newcommand{\vap}{\vec{a'}}
\newcommand{\vas}{\vec{\opt{a}}}
\newcommand{\vb}{\vec{b}}
\newcommand{\vc}{\vec{c}}

\newcommand{\vd}{\vec{d}}
\newcommand{\ve}{\vec{e}}
\newcommand{\vf}{\vec{f}}
\newcommand{\vp}{\vec{p}}

\newcommand{\vfhat}{\vec{\hat{f}}}
\newcommand{\vg}{\vec{g}}
\newcommand{\vk}{\vec{k}}
\newcommand{\vi}{\vec{i}}
\newcommand{\vm}{\vec{m}}
\newcommand{\vo}{\vec{o}}
\newcommand{\vq}{\vec{q}}
\newcommand{\vr}{\vec{r}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vv}{\vec{v}}
\newcommand{\vvp}{\vec{v'}}
\newcommand{\vvs}{\vec{\opt{v}}}
\newcommand{\vw}{\vec{w}}
\newcommand{\vh}{\vec{h}}
\newcommand{\vwhat}{\vec{\hat{w}}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vxp}{\vec{x'}}
\newcommand{\vxs}{\vec{\opt{x}}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vyp}{\vec{y'}}
\newcommand{\vz}{\vec{z}}
\newcommand{\valpha}{\bm{\alpha}}
\newcommand{\vdelta}{\bm{\delta}}
\newcommand{\vDelta}{\bm{\Delta}}
\newcommand{\vepsilon}{\vec{\epsilon}}
\newcommand{\veta}{\vec{\eta}}
\newcommand{\vlambda}{\vec{\lambda}}
\newcommand{\vsigma}{\boldsymbol{\sigma}}
\newcommand{\vmu}{\boldsymbol{\mu}}
\newcommand{\vmuhat}{\vec{\hat{\mu}}}
\newcommand{\vmup}{\vec{\mu'}}
\newcommand{\vnu}{\vec{\nu}}
\newcommand{\vomega}{\vec{\omega}}
\newcommand{\vphi}{\vec{\phi}}
\newcommand{\vpi}{\vec{\pi}}
\newcommand{\vvarphi}{\vec{\varphi}}
\newcommand{\vtheta}{\Theta}
\newcommand{\vthetahat}{\vec{\hat{\theta}}}
\newcommand{\vxi}{\vec{\xi}}
\newcommand{\mzero}{\mat{0}}
\newcommand{\mA}{\mat{A}}
\newcommand{\mB}{\mat{B}}
\newcommand{\mBs}{\mat{\opt{B}}}
\newcommand{\mC}{\mat{C}}
\newcommand{\mD}{\mat{D}}
\newcommand{\mF}{\mat{F}}
\newcommand{\mH}{\mat{H}}
\newcommand{\mI}{\mat{I}}
\newcommand{\mIn}{\mat{I}_n}
\newcommand{\mK}{\mat{K}}
\newcommand{\mL}{\mat{L}}
\newcommand{\mCalL}{\mat{\mathcal{L}}}
\newcommand{\mM}{\mat{M}}
\newcommand{\mP}{\mat{P}}
\newcommand{\mQ}{\mat{Q}}
\newcommand{\mT}{\mat{T}}
\newcommand{\mU}{\mat{U}}
\newcommand{\mV}{\mat{V}}
\newcommand{\mW}{\mat{W}}
\newcommand{\mX}{\mat{X}}
\newcommand{\mLambda}{\bm{\Lambda}}
\newcommand{\mSigma}{\bm{\Sigma}}
\newcommand{\mSigmap}{\bm{\Sigma'}}
\newcommand{\rG}{\rvec{G}}
\newcommand{\rQ}{\rvec{Q}}
\newcommand{\rU}{\rvec{U}}
\newcommand{\rV}{\rvec{V}}
\newcommand{\rX}{\rvec{X}}
\newcommand{\rXp}{\rvec{X'}}
\newcommand{\rY}{\rvec{Y}}
\newcommand{\rZ}{\rvec{Z}}
\newcommand{\sA}{\set{A}}
\newcommand{\sB}{\set{B}}
\newcommand{\sC}{\set{C}}
\newcommand{\sD}{\set{D}}
\newcommand{\sI}{\set{I}}
\newcommand{\sM}{\set{M}}
\newcommand{\sS}{\set{S}}
\newcommand{\sU}{\set{U}}
\newcommand{\sX}{\set{X}}
\newcommand{\sY}{\set{Y}}
\newcommand{\sZ}{\set{Z}}
\newcommand{\spA}{\spa{A}}
\newcommand{\spB}{\spa{B}}
\newcommand{\spC}{\spa{C}}
\newcommand{\spD}{\spa{D}}
\newcommand{\spH}{\spa{H}}
\newcommand{\spP}{\spa{P}}
\newcommand{\spQ}{\spa{Q}}
\newcommand{\spT}{\spa{T}}
\newcommand{\spX}{\spa{X}}
\newcommand{\spZ}{\spa{Z}}
\newcommand{\fs}{\opt{f}}
\newcommand{\ps}{\opt{p}}
\newcommand{\qs}{\opt{q}}
\newcommand{\xs}{\opt{x}}
\newcommand{\ys}{\opt{y}}
\newcommand{\Bs}{\opt{B}}
\newcommand{\Qs}{\opt{Q}}
\newcommand{\sSs}{\opt{\sS}}
\newcommand{\hQs}{\opt{\hat{Q}}}
\newcommand{\Vs}{\opt{V}}
\newcommand{\pis}{\opt{\pi}}

%--------Superquadrics--------
\newcommand{\scalex}{s_x}
\newcommand{\scaley}{s_y}
\newcommand{\scalez}{s_z}
\newcommand{\scale}{\vec{s}}
\newcommand{\shape}{\epsilon}
\newcommand{\exponent}{\epsilon}
\newcommand{\quaternion}{\vec{q}}
\newcommand{\q}{\vec{q}}
\newcommand{\translation}{\vec{t}}
\newcommand{\exist}{\alpha}
%\newcommand{\shape1}{\epsilon_1}
%\newcommand{\shape2}{\epsilon_2}



\newcommand{\pc}{\mathcal{P}}
\newcommand{\NumPrim}{P}
\newcommand{\NumPoints}{N}
\newcommand{\NumSampledPoints}{S}
\newcommand{\HiddenDim}{H}
\newcommand{\AssignMatrix}{M}
\newcommand{\AssignMatrixEl}{m}
\newcommand{\PointFeatures}{\mathcal{F}_{PC}}
\newcommand{\SQFeatures}{\mathcal{F}_{SQ}}
\newcommand{\Loss}{\mathcal{L}}
\newcommand{\ReconstructionLoss}{\mathcal{\Loss}_{rec}}
\newcommand{\ParsimonyLoss}{\mathcal{\Loss}_{par}}
\newcommand{\NorLoss}{\mathcal{\Loss}_{N}}
\newcommand{\PCSQLoss}{\mathcal{\Loss}_{\pc\rightarrow SQ}}
\newcommand{\SQPCLoss}{\mathcal{\Loss}_{SQ\rightarrow \pc}}
\newcommand{\ExistLoss}{\mathcal{\Loss}_{exist}}
\newcommand{\wpar}{\lambda_{par}}
\newcommand{\wexist}{\lambda_{exist}}


\newcommand{\circlenum}[1]{{\textcircled{\scriptsize{#1}}}}
\usepackage[dvipsnames]{xcolor}
\usepackage{url}
\newcommand{\drad}{d_r}

\newcommand{\elisabetta}[1]{{\color{magenta} {\textbf{[#1}} --~\textit{Elisabetta}\textbf{]}}}

